Examining the Effects of Immersive and Non-Immersive Presenter Modalities on Engagement and Social Interaction in Co-located Augmented Presentations

Head-worn augmented reality (AR) allows audiences to be immersed and engaged in stories told by live presenters. While presenters may also be in AR to have the same level of immersion and awareness as their audience, this symmetric presentation style may diminish important social cues such as eye contact. In this work, we examine the effects this (a)symmetry has on engagement, group awareness, and social interaction in co-located one-on-one augmented presentations. We developed a presentation system incorporating 2D/3D content that audiences can view and interact with in AR, with presenters controlling and delivering the presentation in either a symmetric style in AR, or an asymmetric style with a handheld tablet. We conducted a within- and between-subjects evaluation with 12 participant pairs to examine the differences between these symmetric and asymmetric presentation modalities. From our findings, we extracted four themes and derived strategies and guidelines for designers interested in augmented presentations.

==> sections/TranscriptAnalysis-mc.tex <==


Engaged with map/content - au01, au02, au03, au04, au05, au06, au07, au08, au09, au11, au12
- focusing on content / map
o hearing more than seeing the presenter (presenter as narrator, voice-over) - au01, au07, au08, au10 au02 
* (liked presenter keep going and talking) – au02
* just let presenter to do what they do but focus on their own thing – au05
o wasn’t paying attention to presenter – au06, au07
o did not have much eye contact with presenter – au04
* au04 wants to replace presenter by avatar (more focus on the data and virtual)
o because presenter was off on the side in a large area versus in the center – au07, au10
o interaction cue as a way to know engagement – pr03, pr05
- fully immersed with data / new perspective of data - au03, au08, au11, pr02
o Live data vis is better than excel sheet - au11
* Eye and brain sync, number starts to make sense
- perception of visualized data didn’t align with what was expected – au07, au08, au12
- dynamic changes (of the data points) across the presentation captured my interest – au04, au11, au12
o showing chart in VR make people grasp much faster than explaining in powerpoint or in email – au11
- most engagement content among the four times in life – au06
Concerned that audience seem to be distracted by the map – pr01, pr03, pr04
* expect audience to just look at me
Engaged with both content and presenter - au03, au04, au06, au08, au09, au11
- presenter asked questions about interest, customized experience helped – au04, au09
- presenter guided their attention to different parts – au06, au09
- presenter’s walkthrough the data story was helpful – au08
- interacted with presenter and they speak out the content – au11

Had Eye Contact, au03, au04, au06, pr05, au11
- feel that their eyes cannot be seen (uni-directional) - au03
- goggle restricted my peripheral view – au06, au12, au08
o needed to step back to see the entire desk/map – au06, au08
o size of vis going outside of vision – au08, pr01
- have audience captured can help shy presenter? – au11
- headset is a bit burden for audience to rotate head or look at partner – au11, pr03, pr06
- track the eye focus of audience in headset – pr04
- eye contact as necessary for social engagement
o seeing eye and facial expression/eye movement is extremely important – au11
o eye contact makes the user feel connected and showing/knowing eye activity is useful - au03, pr05
o try to have eye connected to the presenter to catch what they are talking about  - au11
look at audience’s body language while using tablet  – pr03
had problem have eye contact
- couldn’t see faces (audience wearing headset)– pr05
- couldn’t see presenter, saw but the presenter seems opaque. – au10
o expected an avatar or some way to make it visible
- concerned when the audience is not looking at them – pr01
Had verbal reference of objects with presenter - au02, au03, au05, au06, au09, au12
- verbal reference worked but took some effort - au03
- verbal communication is necessary (especially without eye contact) - au03
- verbal reference didn’t work well as the audience doesn’t know where to look when presenter talks without pointing. – au05
- did not have much verbal reference but assumed the presenter knows (the referenced object) – au06
- verbal comm is a backup - communication helped when presenter had issue using pointer – au06
- mostly verbal reference by calling out name and region of the map – au09, au12, pr05
o don’t know how to point when there are so many cylinders - au09, pr06
* prefer eye tracking for better / con pointing – au09, pr05
o did not use pointer as the presenter wants to practice traditional way – pr05
o having hand point together was helpful – pr05?

Freeform exploration, enjoyed less controlled by presenter - au01, au03, au05, au06, pr05
- had control conflict / compete for control - au01, au05, au06, pr04
o au05 avoid competition by not touching the map but just pointing
o need turn-based control, dedicated window for audience to get control - au01,  pr01
o presenter gives some time for  each slide to let audience explore on their own is great (it takes time to consume large amount of info)- au03
o would try to avoid competing by letting one do it – au06
o pr01 – compete for map, jumpy manipulation in headset
o wish to reset the map after audience move – pr04
o divide the quadrants to help focus (for better collaboration) – au06
- (during exploration) visual cue letting people know about where to focus to avoid throw off – au06
- the audience can just quietly click on things to figure out the answers without breaking presenter’s flow, and wish for automated feature like that too – au06
o interactive glossary for people to explore
o have your own screen for your own exploration
- desire for more freedom
o I could do whatever I want to do – au07
* Want more control, even go back of the slides
o Did search for cities together but control was led by presenter – au08
o Wished to have more control since the button click wasn’t working well – au12, pr06

Engaging by asking questions and seeing what they ask about – PR01, pr06

Point at object / zoom to enlarge as main referential method - au01, au02, au03, au04, au05, au06, au07, au08, pr02, au10, pr01, pr03, pr04, pr05
- want more accurate pointing - au03, pr03, pr05
o wish to have eye pointing
- pointed at map in silence but try to collaborate with the presenter - au05
- used controller as laser point – au06
- wish to leave some markers beyond pointing – au07
- point on tablet is more comfortable than controllers – pr02, pr03
- Presenter was pointing out for them – au11
- Pointing was helpful and highlight was easy – pr01
- Switch between zoom and point on tablet is a bit hard – pr01

Aware of partner
- knows the partners is able to see what they are seeing - au02, au03, au06, pr02
o aware of presenter knows where the view is at – au06, au09
- desire for activity visualization for presenter (e.g., eye activity)- au03, pr01
- saw audience’s view and reaction clearly while using tablet, but not paying much attention to audience – pr02?
o Know audience engagement via dialogue and their map interaction – pr02
Lack of awareness - Not sure if they are looking at highlight pointers, or in their own world– pr01, pr04 (tablet-only)
- Have to switch a lot to inspect the other’s view
- Did not know presenter can see what they see – au07


Interface Preference
- Flexibility & reliability of tech - prefers tablet for presenter, flexibility and sense of security / reliability (tablet as robust tech) - au03, pr01
- No preference - audience didn’t see impact from presenter’s interface – au04
- Tablet as easy / familiar interface – PR02, pr01, pr03, pr05, pr06
- Controllers are uncomfortable and weird but got used to it. – pr02, pr03, pr06
o Slower interaction – pr06
- Tablet provides more (social) interactivity and engagement – PR02, pr01, pr03, pr05, pr06
o Tablet seems to make them more talkative – pr01
o More natural conversation in headset – pr04
o Easy to tell audience engagement in tablet – pr06
- VR system takes more brain power – PR02, pr03, pr05
o Being immersed was overwhelming, harder to focus on things – pr05
- Headset version felt more intimate because you can adjust layout – PR02
- Tablet has more anonymity, while headset you are the driver guiding them – pr05
- In headset, natural gestures didn’t come across as directly compared to tablet – pr01, pr05
o Didn’t have the expected level of control, jarred the audience – pr05
o Pointing is more straightforward in AR, especially for 3D – pr04
- Less space for gesture in tablet – pr04
- Better overview / vision in tablet– pr01, pr06
o Speaker notes are hard to read in headset – pr01, pr05
o Less multitasking in tablet – pr05
o Hard to see partner and notes all at once in headset – pr01, pr03, pr05, pr06
- Headset like physical blocker for social interaction – pr03, pr05
- Headset is more collaborative and natural, tablet easier for presenting / operate – pr01, pr04, pr05
o Feel like a presenter while holding tablet– pr05
- See body language better to gauge engagement in headset – pr04
- Less social interaction in tablet, more separate – pr04

Co-presence: 
- audience prefers equal status, stronger sense of doing together (headset) - au01, au02
- AR for co-located, VR for remote - au03
- Had some issue at the beginning knowing where the presenter is referred to or talking about – au05
- In one’s own world (due to asymmetric setup) – au07
- Wish for fully immersive environment and collaboration with avatar – au10
- Ar-ar provides the sense of looking at exactly same thing – pr04

Comparison with power point:
- more dynamism (feedback, encourage more Q&A) - au01, pr05
o encourage Q&A, need more time for people to talk - au04, pr01
o more custom exploration
- expressive visuals, colors and 3D - au01, au02, au03, au12, pr04, pr06
- static slides are boring, refreshing way of taking information - au02 (presenter read-off in headset is better than on static slides)
- it will engage people better than powerpoint because of the interactivity, never fall asleep– au05
- current state is better than existing presentation – au04

Reason / Willing to use the system
- will use the system au01, au02
- wish to have both 2D and 3D as different visualization have different effectiveness, and different acceptance for people - au03, au09
o more link / integration between map and slide – au06
- want easy authoring tool to quickly create 3D presentation - au03 , pr05
o want to map any data from 2d to 3d – au04
o have some standard patterns or nice framework for slides that anyone can use – pr05
o need skills and time to do 3d vis – pr05
- good for small focus groups – au05
- blurry display makes it hard to use for realworld – au07
- if access is not a problem, will use – au09
- if physical interaction is more mature and device being more comfortable, will use it – au12
- could imagine use it for real-life data storystelling– au11
- need some improvement before using – pr03

General usability:
- want lighter headset - au02
- better accessibility – au04
- disorienting - a bit too distributed / sparse surfaces (overlapping each other?) content at different places – au05, au10
o need to move head quite often – au05, pr01, pr03
- desire for augmented pictogram of what the presenter is referring to – au06
- want better opacity and color contrast, better resolution of map - au03 
o want more stable graphics – au04
o contrast with highlight color and neutral color – au05, au09, pr05
o better color, right all gray – au06
o more colorful – au11
- want more immersive (panoramic) experience – au04
- want easier control - au02, au03, au04
o au04 - map jump back, sometimes unpredictable, would be better to have finger manipulation
o single / separate hand interaction and function – au04, au05
* one hand do one thing – au05
- want remote feature, a must – au06
- want better preview between scene slides
- visualization doesn’t match understanding – au05
- wish to be able to google / investigate on the side – au07
- headache / dizzy – pr01, au12



==> sections/TranscriptAnalysis-mg.tex <==
,,,,A,S,A,S,S,A,A,S,A,S,S,A,,,,,,
Theme,Sub Theme,Big Code,Code,AU1,AU02,AU03,AU04,AU05,AU06,AU07,AU08,AU09,AU10,AU11,AU12,PR01,PR02,PR03,PR04,PR05,PR06
,Audience engagement with presenter interpersonally,Social cue expression restricted,"uncertainty if other person can properly see own gestures, references",,,,,,,,,,,,,x,,,,,
,,,Did not do much social interaction,,,,,x,x,,,,,,,,,,x,,
,,,social cues blocked by wearing own headset,,,x,,,,,,,,,,x,,x,,,
,,,nuances of movement missing with the AR pointing,,,,,,,,,,,,,,,x,,,
,,Social cue expression maintained,,,,,,,,,,,,,,,,,,,
,,Social cue observation restricted,Could not see partner’s social cues due to partner's headset,,,x,,,,,,,,,,,,,,,x
,,,less direct interaction in AR version b/c couldn’t see audience,,,,,,,,,,,,,,,x,,,
,,,Did not look at partner at all due to engaging with virtual content,,x,,,,,,,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,,Social cue observation maintained,looked under headset to look at partner,,,,,,,,x,,,,,,,,,,
,,,"importance of seeing the other person’s face, hands, feet (whole body)",,,,,,,,,,x,x,,,,,,,
,,Presenter behaviors actively engaging the audience,presenter's verbal communication/style was engaging,,x,,,,,,,,,,,,,,,,
,,Desire different social cue display,"idea to overlay avatar on presenter's physical face to make them more part of the presentation environment, increase social cues",,,,x,,,,,,,x,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,Audience engagement with virtual content (map),Interactivity was engaging,"interaction leading to creativity, open-ended presentation; this was engaging",x,,,,x,,,,,,,,,,,,,
,,,"interaction = good, engaging",x,,,,x,,,,x,x,x,,,,,,,
,,,presenter's map interaction = engaging,,x,,,,,,,,,,,,,,,x,x
,,Data viz was engaging,"enjoy data viz, map engaging",x,,,,x,,x,x,,x,x,x,,,,,,
,,,dynamic content = engaging,x,,,,x,x,,x,,x,x,x,,,,x,,x
,,,Interesting to link/integrate slide content (2D viz) with 3D viz,,,,,,,x,,x,x,,,,,,,,
,,,adding context to 3D viz made it more engaging,,,,,,,,x,x,,,x,,,,,,
,,3D was engaging,"3D is novel, interesting, engaging",,x,,,,,,,,,,,,x,,,,x
,,,"3D provide different understanding of data, different perspectives",,,x,,,x,,x,,,,,,,,,,
,,,experience / immersion / presence in 3D graphics environment leading to engagement,,,x,,,,,,,,,,,,,,,
,,,3D easy to understand,x,,,,x,x,,,,,,x,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,Audience engagement with both presenter and virtual content,Simulateneous presenter + content engagement,engaged evenly with presenter and content,,,,,,,,x,,,,,,,,,,
,,Effects of engagement with presenter/content on other,interaction leading to more verbal communication with presenter,x,,,,,,,,,,,,,,,,,
,,,presenter out of FOV correlating/leading to more focus on 3D map,,,,,,x,x,,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,Presenter strategies/abilities for driving engagement with content,Directing attention strategies,,,,,,,,,,,,,,,,,,,
,,Presenter ability to engage,familiarity of tablet allowed for more engaging presentation,,,,,,,,,,,,,,x,,,x,x
,,,more dialogue/audience interaction with tablet,,,,,,,,,,,,,,x,,,,
,,,use dialogue to gauge the engagement of the audience,,,,,,,,,,,,,,x,,,,
,,,"speaker notes were distracting, prevented interaction with audience in AR version",,,,,,,,,,,,,,,x,x,,x
,,,map interaction to engage the audience,,,,,,,,,,,,,,,x,,,
,,Presenter understanding of audience engagement,judged engagement based on audience interaction with map,,,,,,,,,,,,,,,x,x,x,
,,,easier to look at and judge engagement in tablet version b/c easier to see audience whole body,,,,,,,,,,,,,,,x,,,
,,,easier to judge engagement in symmetric interaction (don’t have to spend extra effort understanding the other person’s attention),,,,,,,,,,,,,,,,x,,
,,,,,,,,,,,,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,Presenter preferences,Advantages of tablet,tablet was more efficient to use,,,,,,,,,,,,,,x,x,,,
,,,tablet provides more flexibility,,,,,,,,,,,,,,,x,,,
,,,tablet provides easier control,,,,,,,,,,,,,,,x,,,
,,,"would use tablet, not AR version",,,,,,,,,,,,,,,x,,,
,,,enjoyed being able to position the presentation notes,,,,,,,,,,,,,,x,,,,
,,,,,,,,,,,,,,,,,,,,,
,Freedom of exploration,Appreciated being able to explore,freedom / control of presentation experience = good,x,,,,,,,,,,,,,,,,,
,,Wanted more exploration ability,desire for separate spaces or private window to display / look up related content,,,,,,x,x,,,,,x,,,,,,
,,Conflict of control between presenter and audience,conflict of control between when interacting with map; confusing or problematic,x,,,,,x,x,,,,,,,,,,,
,,Difference in sense of control,Audience deferred control to the presenter,,,,x,x,,,,,,,,,,,,,x
,,,Audience did not want to mess up the presenter by moving the map,,,,,,,x,x,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,Co-Presence,Feeling together,experiencing the presentation together with the other person,,x,,,,,,,,,,,,,,x,,
,,,"symmetric felt more intimate, connected",,,,,,,,,,,,,,x,,x,,
,,Feeling apart,having two separate experiences,,,,,,,x,,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,General usability,Ergonomic issues,difficulty moving head to look at all virtual content,,,,x,,x,,,,,,x,,,,,,
,,,"Too much physical movement, discomfort (e.g. neck strain) when using headset",,,,,x,,,,,,x,,,,x,,,
,,Technical issues,"technical issues being distracting, prevent total understanding of presenter's references",,x,,,,,,,,,,,,,,,,x
,,Require adaptation to new system,difficulty adapting to new system,,x,,,,x,x,,,,,,,x,,x,,x
,,Usability issues,desire for more intuitive controls,,x,,,,,,,,,,,,,,,,
,,,desire for hand tracked interaction,,,,,,x,,,,,,,,,,,,
,,,difficult to use VR headsets with everyone (accessibility issues),,,,x,,,x,,,,,,,,,,,
,,,difficult to switch between modes (annotation/map interaction),,,,,,,,,,,,,,,,,,
,,,too focused on giving presentation to move speaker notes,,,,,,,,,,,,,,,x,,,
,,Usability positives,would use this system,,x,,,,,,x,x,x,x,,x,x,,,,
,,,AR good for co-located scenario,,,x,,,,,,,,,,,,,,,
,,,tablet allows more freedom of movement,,,x,,,,,,,,,,,,,,,
,,,tablet seems more robust platform; using them together makes system feel more robust,,,x,,,,,,,,,,,,,,,
,,,enjoyed walking around in the physical space,,,,,,,,x,,,,,,,,,,
,,,"would use with small number of people, e.g. < 5",,,,,,,,x,,,,,,,,,,
,,,meetings can be made more efficient with this system,,,,,,,,,,,x,,,,,,,
,,,tablet provides familiar interface,,,,,,,,,,,,,,x,x,,,
,,Confusion with data viz,surprised at data viz content (how tall LA was),,,,,,,x,,,,,,,,,,,
,,,,,,,,,,,,,,,,,,,,,
,Inter-referential awareness,Difficulty with references,"desire for more attention cues to be shared (gaze, hands, etc.)",x,,x,,,,,,,,,,,,,,,
,,,difficult to understand what partner is looking at / referring to,,,,,,x,,,,,,,,,,,,
,,,desire for grounding in global positioning/reference,x,,,,,,,,,,,,,,,,x,x
,,,unsure what partner was looking at,,,,,,,,,,x,,,,,,,,
,,,dense data points cause difficulty with references,,,,,,,,,x,,,,,,,,,
,,Referencing strategies,Using verbal communication for references,,x,,,,x,,,x,,x,x,,,,,x,
,,,using virtual rays to easily refer to virtual content,,,,x,x,x,,x,,,x,,,,x,,,
,,,virtual rays familiar way to refer to content (laser pointer),,,,,,x,,,,,,,,,,,,
,,,multiple perspectives helped presenter tell what audience attended to,,,,,,,,,x,,,,,,,,,
,,,map interaction to direct the audience’s attention,,,,,,,,,,,,,,x,x,,,
,,,Presenter use tablet pointer to refer to objects,,,,,,,,,,,,,,,x,x,,
,,,easy to make references in symmetric interaction,,,,,,,,,,,,,,,,x,,
,,,,,,,,,,,,,,,,,,,,,
,,,more natural to make social gestures in symmetric,,,,,,,,,,,,,,,,x,,
,,,asymmetric interaction space leading to difficulty in judging attention/engagement,,,,,,,,,,,,,,,,x,,
,,,2D audience view on tablet less reliable than symmetric 3D view,,,,,,,,,,,,,,,,x,,
,,,two separate experiences in tablet version,,,,,,,,,,,,,,,,x,,
,,,tablet pointer added too much overhead,,,,,,,,,,,,,,,,,x,
,,,wanted AR mode for tablet to see AR view of space,,,,,,,,,,,,,,,,,x,
,,,"being immersed was overwhelming, distracting from presentation script/story",,,,,,,,,,,,,,,,,x,
,,,"to presenter, symmetric felt like they were in control of the presentation, asymmetric allowed more audience exploration",,,,,,,,,,,,,,,,,x,
,,,"felt like leading own experience in AR version, audience along for the ride",,,,,,,,,,,,,,,,,x,
,,,used audience live view to judge their attention,,,,,,,,,,,,,,,,,,x
,,,easier to judge engagement in asymmetric b/c of live view,,,,,,,,,,,,,,,,,,x
,,,judged engagement based on audience social interaction,,,,,,,,,,,,,,,,,,x


==> sections/old_files/04_results_01_quant_1.0_OLD.tex <==
\section{\changetext{Questionnaire and Observational Data}}
In this section, we first present the responses to the post-study questionnaire and a summary of participant behaviors we observed.
Due to the nature of this study as exploratory research intended to inform future research on immersive presentation systems
% and our small sample size ($n = 6$ groups for each experimental condition), 
we report descriptive statistics about our quantitative data without statistical test results~\cite{vornhagen2020stat}.
% \newtext{Unless otherwise noted in this section, we did not find any trends related to presenters' presentation experience.}
\newtext{We report only the most relevant results in this section.
For a more detailed look at all of the quantitative results, refer to~\autoref{sec:appendix}.}

\begin{figure}[t]
    \centering
    \newcommand{\subfigwidth}{0.3\textwidth}
    % First subfigure
    \begin{subfigure}{\subfigwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tlx_box_3.pdf}
        \caption{Presenter Cognitive Load}
        \label{fig:tlx}
    \end{subfigure}
    \begin{subfigure}{\subfigwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/aware_box_2.pdf }
        \caption{Group Awareness}
        \label{fig:awareness}
    \end{subfigure}
    \begin{subfigure}{\subfigwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/engage_box_2.pdf}
        \caption{Engagement}
        \label{fig:engagement}
    \end{subfigure}
    % Description
    % (a) Box plot with Cognitive Load on the y-axis and NASA-TLX Sub-Scale on the x-axis. Three groups of x-axis boxes: Mental, Physical, and Performance sub-scales. Two boxes in each pair with different colors: aymmetric as light blue and symmetric as darker blue.
    % (b) Box plot with Group Awareness on the y-axis and Presenter Modality on the x-axis. Two groups of x-axis boxes based on Presenter Modality: asymmetric and symmetric. Two boxes in each pair with different colors: Audience as yellow and Presenter as muted blue.
    % (c) Box plot with Engagement on the y-axis and Presenter Modality on the x-axis. Two groups of x-axis boxes based on Presenter Modality: asymmetric and symmetric. Two boxes in each pair with different colors: Audience as yellow and Presenter as muted blue.
        \caption{Box plots for questionnaire responses.
        (a) Average presenter scores for the mental demand (lower is easier), physical demand (lower is easier), and performance (higher is better) categories of the NASA-TLX~\cite{hart2006tlx}.
        (b) Average scores for questions about group awareness (see~\autoref{tab:awareness}).
        Points represent individual participant responses and are colored by presentation group and presenter: within a presenter modality, points of the same color represent participants in the same presentation session; across presenter modalities, points of the same color represent the same presenter participant.
        (c) Average scores for questions about the presenter's ability to engage the audience in the presentation and the audience's ratings of their engagement in the presentation (see~\autoref{tab:engagement}).
        Points represent individual participant responses and are colored by presentation group and presenter.
        }
    \label{fig:questionnaires}
\end{figure}

\subsection{Questionnaire Responses}
In this section, we report the results of the questionnaires described in~\autoref{sec:methods:q}.
All questionnaire responses are on a 7-point Likert scale.
These results are visualized in~\autoref{fig:questionnaires}.

\paragraph{Cognitive Load.}
\changetext{
On the NASA-TLX cognitive load questionnaire, presenters reported a slightly higher mental demand score for the symmetric presentation modality (Mdn.: $3.50$; IQR: $2.50$, $2.25 - 4.75$) compared to the asymmetric modality (Mdn.: $3.00$; IQR: $2.25$, $1.50 - 3.75$).
}
% \changetext{
% Presenters reported similar physical demand scores for both the symmetric modality (Mdn.: $2.50$; IQR: $2.50$, $1.25 - 3.75$) and asymmetric modality (Mdn.: $2.50$; IQR: $1.75$, $1.25 - 3.00$).
% Presenters reported similar performance scores for the symmetric modality (Mdn.: $5.50$; IQR: $0.75$, $5.25 - 6.00$) and the asymmetric modality (Mdn.: $5.50$; IQR: $1.75$, $5.00 - 6.75$).
% }

%%% PREVIOUS:
% For the symmetric presentation modality, presenters reported a median mental demand score (higher is more demanding) of $3.50$ (IQR: $2.25 - 4.75$).
% For the asymmetric modality, presenters reported a median mental demand score of $3.00$ (IQR: $1.50 - 3.75$).
% For the symmetric modality, presenters reported a median physical demand score (higher is more demanding) of $2.50$ (IQR: $1.25 - 3.75$).
% For the asymmetric modality, presenters reported a median physical demand score of $2.50$ (IQR: $1.25 - 3.00$).
% For the symmetric modality, presenters reported a median performance score (higher is better) of $5.50$ (IQR: $5.25 - 6.00$).
% For the asymmetric modality, presenters reported a median performance score of $5.50$ (IQR: $5.00 - 6.75$).
% % \newtext{We did not observe any tendencies related to presenters' presentation experience.}

% Presenters reported their average mental demand (higher is more demanding) as $3.67$ ($SD = 2.16$) for presentations in which presenters used the symmetric presentation modality.
% For the asymmetric presentation modality, presenters' average mental demand was $2.83$ ($SD = 1.60$).
% % , and the audience reported their average mental demand as $2.50$ ($SD = 1.87$).
% % , and audience members' average mental demand was $2.5$ ($SD = 1.05$).
% For the symmetric presentation modality, presenters' average physical demand was $2.83$ ($SD = 1.94$).
% For the asymmetric presentation modality, presenters' average physical demand (higher is more demanding) was $2.67$ ($SD = 1.86$).
% For the symmetric presentation modality, presenters' average self-assessed performance was $5.50$ ($SD = 0.84$).
% Presenters rated their performance (higher is better) on average for the asymmetric presentation modality as $5.83$ ($SD = 0.98$).



\paragraph{Group Awareness.}
% Presenter and audience participants both rated their group awareness higher in the symmetric presentation modality (Mdn.: $6.12$; IQR: $0.75$, $5.53 - 6.28$) compared to the asymmetric modality (Mdn.: $5.00$; IQR: $1.07$, $4.59 - 5.66$).
Presenter participants rated their group awareness higher in the symmetric presentation modality (Mdn.: $5.75$; IQR: $2.03$, $4.22 - 6.25$) compared to the asymmetric modality (Mdn.: $5.31$; IQR: $0.72$, $5.00 - 5.72$).
Similarly, audience participants rated their group awareness higher in the symmetric presentation modality (Mdn.: $6.12$; IQR: $0.34$, $6.00 - 6.34$) compared to the asymmetric modality (Mdn.: $4.62$; IQR: $0.38$, $4.53 - 4.91$).

% More specifically, in the symmetric presentation modality, presenters rated their group awareness with the audience with a median score of $5.75$ (IQR: $2.03$, $4.22 - 6.25$), and audience participants rated their group awareness with the presenters with a median score of $6.12$ (IQR: $0.34$, $6.00 - 6.34$).
% For the asymmetric presentation modality, presenters rated their group awareness with the audience with a median score of $5.31$ (IQR: $0.72$, $5.00 - 5.72$), and the audience rated their group awareness with the presenters with a median score of $4.62$ (IQR: $0.38$, $4.53 - 4.91$).

%%% PREVIOUS:
% For the symmetric presentation modality, presenters rated their group awareness with the audience with a median score (higher is better awareness) of $5.75$ (IQR: $4.22 - 6.25$), and audience rated their group awareness with the presenters with a median score of $6.12$ (IQR: $6.00 - 6.34$).
% For the asymmetric presentation modality, presenters rated their group awareness with the audience with a median score of $5.31$ (IQR: $5.00 - 5.72$), and the audience rated their group awareness with the presenters with a median score of $4.62$ (IQR: $4.53 - 4.91$).
% % For the symmetric presentation modality, presenters rated their group awareness with the audience on average as $5.35$ ($SD = 1.41$), and audience rated their group awareness with the presenters on average as $6.21$ ($SD = 0.47$).
% % For the asymmetric presentation modality, presenters rated their group awareness with the audience (higher is better awareness) on average as $5.17$ ($SD = 1.22$), and the audience rated their group awareness with the presenters on average as $4.90$ ($SD = 0.63$).

\paragraph{Engagement.}
\newtext{
% Engagement scores were high overall for both presenter (Mdn.: $6.39$; IQR: $0.59$, $5.97 - 6.56$) and audience participants (Mdn.: $6.28$; IQR: $1.28$, $5.53 - 6.81$).
% Engagement was slightly higher in the symmetric (Mdn.: $6.50$; IQR: $0.81$, $6.08 - 6.89$) compared to the asymmetric modality (Mdn.: $5.94$; IQR: $1.12$, $5.44 - 6.56$).
Presenters' engagement scores were higher for the symmetric modality (Mdn.: $6.39$; IQR: $1.11$, $5.75 - 6.86$) compared to the asymmetric modality (Mdn.: $6.06$; IQR: $1.25$, $5.47 - 6.72$).
Audience participants' engagement scores were higher for the symmetric modality (Mdn.: $6.50$; IQR: $0.53$, $6.36 - 6.89$) compared to the asymmetric modality (Mdn.: $5.94$; IQR: $0.77$, $5.56 - 6.33$).
}
% \newtext{The median of audience participants' scores on the presentation engagement questionnaire (see~\autoref{tab:engagement}) was $6.39$ (IQR: $0.59$, $5.97 - 6.56$).}
% \newtext{The median of presenter participants' scores on the engagement questionnaire was $6.28$ (IQR: $1.28$, $5.53 - 6.81$).}
% \newtext{More specifically, audience participants reported a median score of $6.00$ (IQR: $1.00$, $6.00 - 7.00$) for the \textit{Curiosity} sub-scale of the engagement questionnaire (see ~\autoref{tab:engagement}).}
% \newtext{Presenters reported a median score of $6.00$ (IQR: $2.00$, $5.00 - 7.00$) for the \textit{Curiosity} sub-scale of the engagement questionnaire.}
% \newtext{
% For the Interpersonal sub-scale of the presentation engagement questionnaire (see~\autoref{tab:engagement}), presenters reported approximately the same scores in both symmetric and asymmetric presentation modalities (both with Mdn.: $6.50$; IQR: $1.00$, $6.00 - 7.00$), but audience participants reported slightly higher interpersonal engagement in the symmetric modality (Mdn.: $6.50$; IQR: $1.00$, $6.00 - 7.00$) compared to the asymmetric modality (Mdn.: $5.50$; IQR: $1.00$, $5.00 - 6.00$).
% }
\newtext{Across both modalities, presenters who reported having weekly experience giving presentations tended to rate their ability to engage the audience more highly with a median score of $6.81$ (IQR: $0.17$, $6.72 - 6.89$) compared to $5.61$ (IQR: $0.94$, $5.25 - 6.19$) for those with occasional presentation experience.}

%%% PREVIOUS:
% For the symmetric presentation modality, presenters rated their ability to engage the audience with a median score (higher is better engagement) of $6.39$ (IQR: $5.75 - 6.86$), and audience rated their engagement with the presenters with a median score of $6.50$ (IQR: $6.36 - 6.89$).
% For the asymmetric presentation modality, presenters rated their ability to engage the audience with a median score (higher is better engagement) of $6.06$ (IQR: $5.47 - 6.72$), and audience rated their engagement with the presenters with a median score of $5.94$ (IQR: $5.56 - 6.33$).
% \newtext{Across both modalities, presenters who reported having weekly experience giving presentations tended to rate their ability to engage the audience more highly with a median score of $6.81$ (IQR: $6.72 - 6.89$) compared to $5.61$ (IQR: $5.25 - 6.19$) for those with occasional presentation experience.}



\subsection{\changetext{Observational Data}}
% section for Boris / observed activities summary
In this section, we report quantitative summaries of the behaviors we annotated in the video recordings of the experimental presentation sessions.

\subsubsection{Social Interaction}

\begin{figure}[t]
    \centering
    \newcommand{\subfigwidth}{0.28\textwidth}
    % \newcommand{\subfigwidth2}{0.125\textwidth}
    % First subfigure
    \begin{subfigure}{\subfigwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/expr_box_2.pdf}
        \caption{}
        \label{fig:socialexpr_pid}
    \end{subfigure}
    \hspace{3ex}
    \begin{subfigure}{\subfigwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/lookat_box_2.pdf}
        \caption{}
        \label{fig:lookat}
    \end{subfigure}
    \hspace{3ex}
    \begin{subfigure}{0.14\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eye_occurrence.pdf}
        \caption{}
        \label{fig:eye_occur}
    \end{subfigure}
    \hspace{3ex}
    \begin{subfigure}{0.14\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eye_percent.pdf}
        \caption{}
        \label{fig:eye_percent}
    \end{subfigure}
    % Description
    % (a) Box plot with Social Expression Count on the y-axis and Presenter Modality on the x-axis. Two groups of x-axis boxes based on Presenter Modality: asymmetric and symmetric. Two boxes in each pair with different colors: Audience as yellow and Presenter as muted blue.
    % (b) Box plot with Percent of Presentation Looking at Partner on the y-axis and Presenter Modality on the x-axis. Two groups of x-axis boxes based on Presenter Modality: asymmetric and symmetric. Two boxes in each pair with different colors: Audience as yellow and Presenter as muted blue.
    % (c) Box plot with Eye Contact Occurrence on the y-axis and Presenter Modality on the x-axis. Two boxes on the x-axis for each Presenter Modality: asymmetric and symmetric.
    % (d) Box plot with Percent of Presentation Making Eye Contact on the y-axis and Presenter Modality on the x-axis. Two boxes on the x-axis for each Presenter Modality: asymmetric and symmetric.
        \caption{Social interactions for each presentation modality. (a) Box plot showing the total number of social expressions (gesturing to each other, nodding at each other, smiling at each other, and laughing) observed for each participant and each presenter modality.
        Points are colored by presentation group and presenter: within a presenter modality, points of the same color represent participants in the same presentation session; across presenter modalities, points of the same color represent the same presenter participant.
        (b) Box plot showing the percentage of presentation time participants looked at each other.
        Points are colored by presentation group and presenter.
        (c) Box plot showing the number of times participants made eye contact during the presentation.
        Points are colored by presentation group.
        (d) Box plot showing the percentage of the presentation during which participants made eye contact (i.e., looked at each other simultaneously).}
    \label{fig:socialinteraction}
\end{figure}

% Asymmetric Audience                                 3.58                     6.83
% Asymmetric Presenter                                4                        6.23
% Symmetric  Audience                                 1.08                     1.51
% Symmetric  Presenter                                1.33                     1.75

\paragraph{Social Expressions}
% \newtext{
% Both presenter and audience participants exhibited a slightly greater number of social expressions in the asymmetric modality compared to the symmetric modality.
% }
\changetext{
Presenters exhibited more social expressions in the asymmetric modality (Mdn.: $1.50$; IQR: $4.50$, $0.00 - 4.50$) compared to the symmetric modality (Mdn.: $0.50$; IQR: $2.50$, $0.00 - 2.50$). 
Audience participants also exhibited more social expressions in the asymmetric modality (Mdn.: $4.50$; IQR: $13.50$, $0.00 - 13.5$) compared to the symmetric modality (Mdn.: $2.50$; IQR: $1.75$, $1.25 - 3.00$).
% In the asymmetric presentation modality, the median number of social expressions exhibited by the presenter was $1.50$ (IQR: $4.50$, $0.00 - 4.50$), and the audience's median number of social expressions was $4.50$ (IQR: $13.50$, $0.00 - 13.5$).
% For the symmetric presentation modality, the median number of social expressions exhibited by the presenter was $0.50$ (IQR: $2.50$, $0.00 - 2.50$), and the median number of social expressions exhibited by the audience was $2.50$ (IQR: $1.75$, $1.25 - 3.00$).
% The number of social expressions observed per participant is shown in~\autoref{fig:socialexpr_pid}.
}

%%% PREVIOUS:
% We observed how many times participants exhibited social expressions during the presentation.
% Participants gesturing to each other, nodding at each other, smiling at each other, and laughing were among the social expressions exhibited.
% For presentations in which the presenter used the symmetric presentation modality, the median number of social expressions exhibited by the presenter was $0.50$ (IQR: $0.00 - 2.50$), and the median number of social expressions exhibited by the audience was $2.50$ (IQR: $1.25 - 3$).
% In the asymmetric presentation modality, the presenter's median social expressions were $1.50$ (IQR: $0.00 - 4.50$), and the audience's median number of social expressions was $4.50$ (IQR: $0.00 - 13.5$).
% % For presentations in which the presenter used the asymmetric presentation modality, the presenter exhibited an average of $4.0$ ($SD = 6.23$) social expressions, and the audience exhibited an average of $3.58$ ($SD = 6.83$ social expressions.
% % In the symmetric presentation modality, the presenter exhibited an average of $1.33$ ($SD = 1.75$) social expressions, and the audience exhibited an average of $1.08$ ($SD = 1.51$) social expressions.
% The number of social expressions observed per participant is shown in~\autoref{fig:socialexpr_pid}.


\paragraph{Time Looking At Partner}
\changetext{
We observed that presenters tended to look at the audience for a greater percentage of the presentation when using the asymmetric modality (Mdn.: $5.65\%$; IQR: $8.30\%$, $1.65\% - 9.95\%$) compared to the symmetric modality (Mdn.: $6.65\%$; IQR: $10.05\%$, $1.15\% - 11.20\%$).
However, we observed the opposite tendency for audience participants: that they looked at the presenter more when using the symmetric modality (Mdn.: $5.45\%$; IQR: $8.20\%$, $3.80\% - 12.00\%$) compared to the asymmetric modality (Mdn.: $2.80\%$; IQR: $4.33\%$, $1.35\% - 5.68\%$).
}
% \changetext{
% For presentations in which the presenter used the symmetric presentation modality, the median percentage of the presentation during which the presenter looked at the audience was $5.65\%$ (IQR: $8.30\%$, $1.65\% - 9.95\%$), and the median percentage of the presentation the audience looked at the presenter was $5.45\%$ (IQR: $8.20\%$, $3.80\% - 12.00\%$).
% For the asymmetric presentation modality, the median presentation duration percentage during which the presenter looked at the audience was $6.65\%$ (IQR: $10.05\%$, $1.15\% - 11.20\%$), and the median percentage of presentation the audience looked at the presenter was $2.80\%$ (IQR: $4.33\%$, $1.35\% - 5.68\%$).
% These results are visualized in~\autoref{fig:lookat}.
% }

%%% PREVIOUS:
% % 1 Asymmetric Audience              4.03      4.12
% % 2 Asymmetric Presenter             7.95      8.41
% % 3 Symmetric  Audience             11.0      13.4 
% % 4 Symmetric  Presenter             5.67      4.86
% We observed how much participants looked at each other during the presentation (as opposed to looking at the virtual presentation content).
% For presentations in which the presenter used the symmetric presentation modality, the median percentage of the presentation during which the presenter looked at the audience was $5.65\%$ (IQR: $1.65\% - 9.95\%$), and the median percentage of the presentation the audience looked at the presenter was $5.45\%$ (IQR: $3.80\% - 12.00\%$).
% For the asymmetric presentation modality, the median presentation duration percentage during which the presenter looked at the audience was $6.65\%$ (IQR: $1.15\% - 11.20\%$), and the median percentage of presentation the audience looked at the presenter was $2.80\%$ (IQR: $1.35\% - 5.68\%$).
% These results are visualized in~\autoref{fig:lookat}.


\paragraph{Eye Contact}
\changetext{
Participants had more occurrences of eye contact in the asymmetric modality (Mdn.: $2.50$; IQR: $3.25$, $0.50 - 3.75$) compared to the symmetric modality (Mdn.: $2.00$; IQR: $3.50$, $1.00 - 4.50$).
Similarly, they spent a slightly longer duration of the presentation making eye contact when using the asymmetric modality (Mdn.: $1.00\%$; IQR: $2.47\%$, $0.18\% - 2.65\%$) compared to the symmetric modality (Mdn.: $0.38\%$; IQR: $2.52\%$, $0.08\% - 2.60\%$).
}
% \changetext{
% In the asymmetric presentation modality, the median number of eye contact occurrences was $2.50$ (IQR: $3.25$, $0.50 - 3.75$).
% In the symmetric presentation modality, the median number of occurrences of eye contact between participants was $2.00$ (IQR: $3.50$, $1.00 - 4.50$).
% These results are visualized in~\autoref{fig:eye_occur}.
% We also computed the percentage of the presentation participants spent making eye contact with each other during the presentation.
% In the asymmetric presentation modality, the median percentage of presentation time spent making eye contact was $1.00$ (IQR: $2.47$, $0.18 - 2.65$).
% In the symmetric presentation modality, the median percentage of presentation time spent making eye contact was $0.38$ (IQR: $2.52$, $0.08 - 2.60$).
% These results are visualized in~\autoref{fig:eye_percent}.
% }

%%% PREVIOUS:
% We observed how frequently and for what duration participants made eye contact (i.e., looked at each other simultaneously) during the presentation.
% In the symmetric presentation modality, the median number of occurrences of eye contact between participants was $2.00$ (IQR: $1.00 - 4.50$).
% In the asymmetric presentation modality, the median number of eye contact occurrences was $2.50$ (IQR: $0.50 - 3.75$).
% These results are visualized in~\autoref{fig:eye_occur}.
% We also computed the percentage of the presentation participants spent making eye contact with each other during the presentation.
% In the symmetric presentation modality, the median percentage of presentation time spent making eye contact was $0.38$ (IQR: $0.08 - 2.60$).
% In the asymmetric presentation modality, the median percentage of presentation time spent making eye contact was $1.00$ (IQR: $0.18 - 2.65$).
% These results are visualized in~\autoref{fig:eye_percent}.

\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/ref_box_2.pdf}
        \caption{}
        \label{fig:ref_box}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/ref_count_box.pdf}
        \caption{}
        \label{fig:ref_count}
    \end{subfigure}
    % Description
    % (a) Box plot with Reference Count on the y-axis and Presenter Modality on the x-axis. Two groups of x-axis boxes based on Presenter Modality: asymmetric and symmetric. Two boxes in each pair with different colors: Audience as yellow and Presenter as muted blue.
    % (b) Two box plots side-by-side with Count Per Presentation on the y-axis and Referencing Behavior on the x-axis. The box plot on the left is for Asymmetric presenter modality, and the plot on the right is for Symmetric presenter modality. Referencing Behavior in each plot is further broken down into Pointing, Deictic, Relative, Property, and Chaining. There are two boxes in each referencing behavior: one for Audience in yellow and one for Presenter in blue.
    \caption{Participant referencing behaviors.
    (a) Box plot of the total number of references participants made during a presentation for each participant and each presenter modality.
    Points represent individual participants and are colored by presentation group and presenter: within a presenter modality, points of the same color represent participants in the same presentation session; across presenter modalities, points of the same color represent the same presenter participant.
    (b) Box plot showing the counts of referencing behaviors observed in a presentation session for each participant type and each presenter modality, including \textit{pointing} to virtual objects, using \textit{deictic} speech (e.g., ``this object''), using \textit{relative} language (e.g., ``to the left''), using a \textit{property} reference (e.g., ``the orange cylinder''), using reference \textit{chaining} (e.g., ``next to the last object referenced'').}
    \label{fig:refs}
\end{figure}


\subsubsection{References}

We observed that presenters tended to make more references in the symmetric modality (Mdn.: $11.50$; IQR: $13.75$, $7.25 - 21.00$) compared to the asymmetric modality (Mdn.: $8.50$; IQR: $6.80$, $4.00 - 10.80$).
Audience participants made references at a similar frequency in both symmetric (Mdn.: $5.50$; IQR: $1.00$, $5.00 - 6.00$) and asymmetric modalities (Mdn.: $7.00$; IQR: $5.25$, $2.50 - 7.75$).

\changetext{
We observed that presenters tended to make more pointing references when using the symmetric presentation modality (Mdn.: $6.00$; IQR: $7.45$, $3.75 - 11.20$) compared to the asymmetric modality (Mdn.: $3.50$; IQR: $6.25$, $1.50 - 7.75$).
Audience members made a similar number of pointing references across both symmetric (Mdn.: $3.00$; IQR: $3.50$, $1.25 - 4.75$) and asymmetric modalities (Mdn.: $4.50$; IQR: $4.00$, $1.75 - 5.75$). 
}

\changetext{
Presenters tended to make more verbal references when using the symmetric presentation modality (Mdn.: $7.00$; IQR: $7.75$, $2.00 - 9.75$) compared to the asymmetric modality (Mdn.: $2.50$; IQR: $4.75$, $2.00 - 6.75$).
Audience members made a similar number of pointing references across both symmetric (Mdn.: $3.00$; IQR: $3.50$, $0.50 - 4.0$) and asymmetric modalities (Mdn.: $2.00$; IQR: $2.75$, $0.25 - 3.00$).
Participants mostly used deictic speech when making these verbal references.
% See~\autoref{fig:ref_box} and~\autoref{tab:ref_type} for more fine-grained breakdowns of the participants' verbal referencing behaviors.
}


%%% PREVIOUS:
% We observed how participants made references to virtual content during the presentation.
% We found that when using the symmetric presentation modality, the median number of times presenters made references was $11.50$ (IQR: $7.25 - 21.00$), and the median number of times audience members made references was $5.50$ (IQR: $5.00 - 6.00$).
% In the asymmetric presentation modality, the median number of times presenters made references was $8.50$ (IQR: $4.00 - 10.80$), and the median number of times audience members made references was $7.00$ (IQR: $2.5 - 7.75$).
% These results are shown in~\autoref{fig:ref_box}.

% We broke down participants' referencing behaviors by the kind of references they made as well.
% We found that the median number of times presenters made references by pointing to virtual content was $6.00$ (IQR: $3.75 - 11.20$) in the symmetric modality and $3.50$ (IQR: $1.50 - 7.75$) in the asymmetric modality.
% The median number of times presenters made references using deictic speech was $5.50$ (IQR: $1.00 - 9.25$) in the symmetric modality and $1.50$ (IQR: $1.00 - 2.00$) in the asymmetric modality.
% The median number of times presenters made references by using relative language was $0.00$ (IQR: $0.00 - 0.75$) in the symmetric modality and $1.00$ (IQR: $0.25 - 1.75$) in the asymmetric modality.
% The median number of times presenters made references by using verbal property references was $0.00$ (IQR: $0.00 - 0.75$) in the symmetric modality and $1.00$ (IQR: $0.25 - 0.75$) in the asymmetric modality.
% The median number of times presenters made references by using verbal reference chaining was $0.00$ (IQR: $0.00 - 0.00$) in the symmetric modality and $0.00$ (IQR: $0.00 - 0.00$) in the asymmetric modality.

% We found that the median number of times audience members made references by pointing to virtual content was $3.00$ (IQR: $1.25 - 4.75$) in the symmetric modality and $4.50$ (IQR: $1.75 - 5.75$) in the asymmetric modality.
% The median number of times audience members made references using deictic speech was $1.00$ (IQR: $0.25 - 1.75$) in the symmetric modality and $1.50$ (IQR: $0.00 - 3.00$) in the asymmetric modality.
% The median number of times audience members made references by using relative language was $0.00$ (IQR: $0.00 - 0.00$) in the symmetric modality and $1.00$ (IQR: $0.00 - 0.00$) in the asymmetric modality.
% The median number of times audience members made references by using verbal property references was $0.00$ (IQR: $0.00 - 0.75$) in the symmetric modality and $0.00$ (IQR: $0.00 - 0.00$) in the asymmetric modality.
% The median number of times audience members made references by using verbal reference chaining was $0.00$ (IQR: $0.00 - 0.00$) in the symmetric modality and $0.00$ (IQR: $0.00 - 0.00$) in the asymmetric modality.
% These results are visualized in~\autoref{fig:ref_count}.

% We found that presenters on average made $7.83$ ($SD = 6.97$) references by pointing to virtual content in each presentation for the symmetric modality, and on average $4.67$ ($SD = 4.41$) references of this kind for the asymmetric modality.
% They on average made $7.00$ ($SD = 7.90$) references by using deictic speech for the symmetric modality, and on average $2.50$ ($SD = 3.27$) references of this kind for the asymmetric modality.
% They on average made $1.17$ ($SD = 2.40$) references by using relative language for the symmetric modality, and on average $1.17$ ($SD = 1.17$) references of this kind for the asymmetric modality.
% They on average made $0.50$ ($SD = 0.84$) references by using verbal property references for the symmetric modality, and on average $1.50$ ($SD = 2.35$) references of this kind for the asymmetric modality.
% They on average made $0.17$ ($SD = 0.41$) references by using verbal reference chaining for the symmetric modality, and on average $0.00$ ($SD = 0.00$) references of this kind for the asymmetric modality.

% We found that audience members on average made $3.83$ ($SD = 3.97$) references by pointing to virtual content in each presentation for the symmetric modality, and on average $4.83$ ($SD = 4.62$) references of this kind for the asymmetric modality.
% They on average made $1.50$ ($SD = 1.87$) references by using deictic speech for the symmetric modality, and on average $1.50$ ($SD = 1.64$) references of this kind for the asymmetric modality.
% They on average made $0.33$ ($SD = 0.82$) references by using relative language for the symmetric modality, and on average $1.00$ ($SD = 2.45$) references of this kind for the asymmetric modality.
% They on average made $0.67$ ($SD = 1.21$) references by using verbal property references for the symmetric modality, and on average $0.17$ ($SD = 0.41$) references of this kind for the asymmetric modality.
% They on average made $0.00$ ($SD = 0.00$) references by using verbal reference chaining for the symmetric modality, and on average $0.00$ ($SD = 0.00$) references of this kind for the asymmetric modality.



==> sections/presenterinterview.tex <==

Interview Questions – Presenter

Workspace Awareness / Functional communication 
1.	Please describe how you made references to virtual objects, or how you directed your partner’s attention to specific virtual objects for each system.  
•	What was straightforward for you when referring to objects? 
•	What was difficult for you when referring to objects? 
o	Can you think of an alternative method you would want to help you make references
Engagement
1.	How and when did you know that the audience was engaged with the presentation? 
2.	For each system, did you engage the audience more with the presentation content or with social interaction? 
a.	How did you engage the audience in the presentation content? 
b.	How did you engage the audience personally/socially? 

Symmetry of Experience
Symmetric
1.	Please describe how you engaged the audience in the presentation when both you and the audience were wearing AR headsets. How did you capture their interest? 
•	What features of the system made it easy/difficult to engage the audience? 
•	How did you gauge the audience’s interest when you were both using the headsets? 
o	What made it easy/difficult to tell if the audience was engaged? 
	(Participant might describe difficulty of reading facial expressions.) 
Asymmetric
2.	Please describe how you engaged the audience in the presentation when you were using the tablet to control the presentation. How did you capture their interest? 
•	What features of the system made it easy/difficult to engage the audience? 
•	How could you tell when the audience was engaged when you were using the tablet to control the presentation? 
o	What made it easy/difficult to tell if the audience was engaged? 
	(Participant might describe difficulty of understanding what the audience was looking at.) 
Comparison
3.	Please describe any differences you experienced between the presentation when you were both wearing headsets compared to when the presenter was using the tablet. 
4.	How did your control of the presentation differ when you were both wearing headsets compared to when the presenter was using the tablet? 
5.	How did your social interactions differ when you were both wearing headsets compared to when the presenter was using the tablet? 
6.	**NOTE: Any other differences to expect? 

General Feedback 
1.	Which presentation system configuration did you prefer? Why? 
2.	What changes or additional features would you like to see made to the presentation systems? 
3.	If you had this kind of system, would you use it? 
4.	Compare this presentation system to other presentation methods, e.g., PowerPoint. 

